Spatio-temporal Multivariate Time Series Forecast with Chosen Variables

Spatio-Temporal Multivariate time series Forecast (STMF) uses the time series of $n$ spatially distributed variables in a period of recent past to forecast their values in a period of near future. It has important applications in spatio-temporal sensing forecast such as road traffic prediction and air pollution prediction. Recent papers have addressed a practical problem of missing variables in the model input, which arises in the sensing applications where the number $m$ of sensors is far less than the number $n$ of locations to be monitored, due to budget constraints. We observe that the state of the art assumes that the $m$ variables (i.e., locations with sensors) in the model input are pre-determined and the important problem of how to choose the $m$ variables in the input has never been studied. This paper fills the gap by studying a new problem of STMF with chosen variables, which optimally selects $m$-out-of-$n$ variables for the model input in order to maximize the forecast accuracy. We propose a unified framework that jointly performs variable selection and model optimization for both forecast accuracy and model efficiency. It consists of three novel technical components: (1) masked variable-parameter pruning, which progressively prunes less informative variables and attention parameters through quantile-based masking; (2) prioritized variable-parameter replay, which replays low-loss past samples to preserve learned knowledge for model stability; (3) dynamic extrapolation mechanism, which propagates information from variables selected for the input to all other variables via learnable spatial embeddings and adjacency information. Experiments on five real-world datasets show that our work significantly outperforms the state-of-the-art baselines in both accuracy and efficiency, demonstrating the effectiveness of joint variable selection and model optimization.

==> tables_figs_tex/different_missing_rate_continue.tex <==
\begin{table*}[ht]
    \centering
    \footnotesize
    \caption{Performance Comparison under Different Missing Rates}
    \label{tab:different_missing_rate_continue}
    \resizebox{0.65\textwidth}{!}{
    \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|}
        \Hline
        \multirow{2}{*}{\textbf{Datasets}} & \multirow{2}{*}{\textbf{Methods}} & \multicolumn{3}{c|}{\textbf{Node Sparsity 25\%}} & \multicolumn{3}{c|}{\textbf{Node Sparsity 50\%}} & \multicolumn{3}{c|}{\textbf{Node Sparsity 75\%}} \\
        \cline{3-11}
        & & MAE & RMSE & MAPE & MAE & RMSE & MAPE & MAE & RMSE & MAPE \\
        \hline
        \multirow{13}{*}{METR-LA} & STID & 5.05 & 10.31 & 17.85 & 5.35 & 10.73 & 18.88 & 5.84 & 11.35 & 20.57 \\ \cline{2-11}
        & DSformer & 4.02 & 7.69 & 11.05 & 4.38 & 8.27 & 12.78 & 4.77 & 9.21 & 14.59 \\ \cline{2-11}
        & MegaCRN & 3.81 & 7.43 & 10.47 & 3.94 & 7.87 & 11.02 & 4.24 & 8.28 & 12.13 \\ \cline{2-11}
        & DCRNN+GPT4TS & 3.78 & 7.41 & 10.72 & 3.98 & 7.91 & 11.61 & 4.15 & 8.16 & 11.93 \\ \cline{2-11}
        & DFDGCN+TimesNet & 3.72 & 7.42 & 10.42 & 3.89 & 7.68 & 11.45 & 4.14 & 8.11 & 11.75 \\ \cline{2-11}
        & MTGNN+GRIN & 3.69 & 7.28 & 10.48 & 3.77 & 7.43 & 11.22 & 4.12 & 8.05 & 11.58 \\ \cline{2-11}
        & FourierGNN+GATGPT & 3.71 & 7.40 & 10.87 & 3.82 & 7.84 & 11.75 & 4.21 & 8.25 & 12.25 \\ \cline{2-11}
        & LGnet & 3.95 & 7.52 & 10.97 & 4.17 & 8.03 & 11.83 & 4.42 & 8.52 & 13.09 \\ \cline{2-11}
        & GC-VRNN & 3.68 & 7.04 & 10.51 & 3.87 & 7.73 & 10.98 & 4.17 & 8.19 & 11.79 \\ \cline{2-11}
        & TriD-MAE & 3.64 & 7.15 & 10.37 & 3.79 & 7.58 & 11.07 & 3.90 & 7.92 & 11.13 \\ \cline{2-11}
        & BiTGraph & 3.61 & 6.74 & 10.25 & 3.69 & 7.32 & 10.79 & 3.74 & 7.63 & 11.04 \\ \cline{2-11}
        & GinAR & 3.56 & 6.55 & 10.12 & 3.61 & 7.14 & 10.42 & 3.70 & 7.39 & 10.71 \\ \cline{2-11}
        & \textbf{ NIP w. pretrain} & \textbf{3.28} & \textbf{6.50} & \textbf{9.27} & \textbf{3.31} & \textbf{ 6.58} & \textbf{9.56} & \textbf{ 3.47} & \textbf{ 7.20} & \textbf{ 9.98} \\
        \hline
        \multirow{13}{*}{AQI} & STID & 18.54 & 31.97 & 45.19 & 20.32 & 34.28 & 48.48 & 22.79 & 36.36 & 55.39 \\ \cline{2-11}
        & DSformer & 17.73 & 28.22 & 44.81 & 19.06 & 30.35 & 48.09 & 20.63 & 33.22 & 52.05 \\ \cline{2-11}
        & MegaCRN & 15.32 & 28.41 & 33.35 & 16.51 & 29.52 & 35.86 & 19.66 & 33.09 & 48.96 \\ \cline{2-11}
        & DCRNN+GPT4TS & 15.14 & 28.48 & 32.18 & 16.82 & 30.83 & 35.24 & 17.82 & 31.99 & 37.22 \\ \cline{2-11}
        & DFDGCN+TimesNet & 14.62 & 26.33 & 29.73 & 15.76 & 29.30 & 32.85 & 17.85 & 30.51 & 38.68 \\ \cline{2-11}
        & MTGNN+GRIN & 14.89 & 27.13 & 33.29 & 16.37 & 30.02 & 37.82 & 17.94 & 31.97 & 39.29 \\ \cline{2-11}
        & FourierGNN+GATGPT & 14.65 & 27.17 & 32.82 & 16.13 & 30.77 & 38.37 & 18.01 & 31.86 & 39.90 \\ \cline{2-11}
        & LGnet & 16.02 & 27.76 & 38.92 & 18.39 & 31.03 & 44.95 & 20.36 & 34.09 & 49.63 \\ \cline{2-11}
        & GC-VRNN & 14.66 & 26.88 & 31.88 & 15.70 & 28.67 & 34.21 & 16.99 & 30.57 & 37.66 \\ \cline{2-11}
        & TriD-MAE & 14.51 & 26.18 & 29.09 & 15.74 & 28.96 & 32.94 & 16.79 & 29.84 & 35.76 \\ \cline{2-11}
        & BiTGraph & 13.85 & 25.79 & 28.94 & 14.52 & 27.45 & 31.36 & 15.62 & 29.01 & 33.58 \\ \cline{2-11}
        & GinAR & 13.72 & 25.51 & 28.27 & 14.33 & 26.81 & 29.56 & 15.39 & 27.96 & 31.86 \\ \cline{2-11}
        & \textbf{ NIP w. pretrain}& \textbf{ 13.41} & \textbf{ 24.48} & \textbf{ 27.51} & \textbf{ 14.10} & \textbf{ 26.09} & \textbf{ 29.03} & \textbf{ 15.21} & \textbf{ 27.83} & \textbf{ 31.80} \\
        \hline
    \end{tabular}
    }
\end{table*}
